Beyond In-Distribution Performance: A Cross-Dataset Study of Trajectory Prediction Robustness

We study the Out-of-Distribution (OoD) generalization ability of three SotA trajectory prediction models with comparable In-Distribution (ID) performance but different model designs. We investigate the influence of inductive bias, size of training data and data augmentation strategy by training the models on Argoverse 2 (A2) and testing on Waymo Open Motion (WO) and vice versa. We find that the smallest model with highest inductive bias exhibits the best OoD generalization across different augmentation strategies when trained on the smaller A2 dataset and tested on the large WO dataset. In the converse setting, training all models on the larger WO dataset and testing on the smaller A2 dataset, we find that all models generalize poorly, even though the model with the highest inductive bias still exhibits the best generalization ability. We discuss possible reasons for this surprising finding and draw conclusions about the design and test of trajectory prediction models and benchmarks.

==> tables/ID_A2_Results.tex <==
\begin{table*}[tbh]
%\vspace{+5pt}
\caption{Result of In-Distribution testing (6-second prediction horizon) in competition setting on Argoverse 2 test set. For all the metrics, lower the better. Inference time is tested on one Tesla T4 GPU with a scenario of 50 agents and 150 map elements.}
\vspace{+5pt}
\centering
    % \begin{tabularx}{6.2in}{c >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X >{\centering\arraybackslash}X | | >{\centering\arraybackslash}X >{\centering\arraybackslash}X}
    %     \Xhline{3\arrayrulewidth}
    %     \multicolumn{1}{c}{\multirow{2}{*}{Model}}&\multicolumn{1}{c}{minADE_{1}} & \multicolumn{1}{c}{minFDE_{1}} & \multicolumn{1}{c}{minADE_{6}} &
    %     \multicolumn{1}{c}{minFDE_{6}} & \multicolumn{1}{c}{\# model} & \multicolumn{1}{c}{inference time}\\
    %     \multicolumn{1}{c}{}& \multicolumn{1}{c}{[m]}&\multicolumn{1}{c}{[m]}&\multicolumn{1}{c}{[m]}&\multicolumn{1}{c}{[m]}&\multicolumn{1}{c}{params [k]}& \multicolumn{1}{c}{[ms]}\\
    %     \Xhline{3\arrayrulewidth}
    %     \multirow{2}{*}{QCNet} &1.702 & 4.309 & 0.643& 1.244 &7600& 120.89\\
    %     &(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)\\
    %     \hline
    %     Forecast-MAE &1.755 & 4.388& 0.801 & 1.409 & 1900 &12.63\\
    %     w fine-tune &(103.1\%)&(101.8\%)&(124.6\%)&(113.3\%)&(25.0\%)&(10.4\%)\\
    %     \hline
    %     \multirow{2}{*}{EP\_Q (ours)} &2.134 & 5.415 & 0.841 & 1.683 & 334 & 5.72\\
    %     &(125.4\%)&(125.7\%)&(131.0\%)&(135.3\%)&(4.4\%)&(4.7\%)\\
    %     \hline
    %     \multirow{2}{*}{EP\_F (ours)} & 1.887 & 4.567  & 0.801 & 1.526 & \multirow{4}{*}{\thead{345 \\(4.5\%)}}&\multirow{4}{*}{\thead{4.66\\ (3.9\%)}}\\ 
    %     &(110.9\%) & (106.0\%) & (124.6\%) & (122.7\%) &&\\
    %     \cline{1-5}
    %     \multirow{2}{*}{EP\_F w flip (ours)} & 1.846 & 4.456 & 
    %     0.786& 1.485& &\\
    %     & (108.5\%) & (103.4\%) & (122.2\%) & (119.4\%)&&\\
    %     \Xhline{3\arrayrulewidth}
    %     \vspace{-1em}
    % \end{tabularx}
    \begin{tabularx}{\textwidth}{l *{4}{>{\centering\arraybackslash}X} | *{2}{>{\centering\arraybackslash}X}}
    \toprule
    \multirow{2}{*}{\shortstack{model}} & minADE$_{1}$ & minFDE$_{1}$ & minADE$_{6}$ & minFDE$_{6}$ & \# model params& inference time\\
        & [m]&[m]& [m] & [m] & [k]& [ms]\\
        \midrule
        \multirow{2}{*}{QCNet \cite{zhou_query_2023}} &1.702 & 4.309 & 0.643& 1.244 &7600& 120.89\\
        &(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        FMAE \cite{cheng_forecast_2023} &1.741 & 4.355& 0.709 & 1.392 & 1900 &12.63\\
        w pre-train &(102.2\%)&(101.1\%)&(110.3\%)&(111.9\%)&(25.0\%)&(10.4\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        FMAE \cite{cheng_forecast_2023} &1.845 & 4.602& 0.727 & 1.427 & 1900 &12.63\\
        w/o pre-train &(108.4\%)&(106.8\%)&(113.1\%)&(114.7\%)&(25.0\%)&(10.4\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}        
        \multirow{2}{*}{EP-Q (ours)} &2.134 & 5.415 & 0.841 & 1.683 & 334 & 5.72\\
        &(125.4\%)&(125.7\%)&(131.0\%)&(135.3\%)&(4.4\%)&(4.7\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        \multirow{2}{*}{EP-F (ours)} & 1.887 & 4.567  & 0.801 & 1.526 & \multirow{4}{*}{\thead{345 \\(4.5\%)}}&\multirow{4}{*}{\thead{4.66\\ (3.9\%)}}\\ 
        &(110.9\%) & (106.0\%) & (124.6\%) & (122.7\%) &&\\
        \cmidrule(lr){2-5}
        \multirow{2}{*}{EP-F w flip (ours)} & 1.846 & 4.456 & 
        0.786& 1.485& &\\
        & (108.5\%) & (103.4\%) & (122.2\%) & (119.4\%)&&\\
        \bottomrule
    \end{tabularx}
    \label{tab: in-distribution result a2}
    \vspace{-5pt}
\end{table*}


==> tables/ID_WO_Results.tex <==
\begin{table*}[tbh]
%\vspace{+5pt}
\caption{Result of In-Distribution testing (4.1-second prediction horizon) on WO validation split. For all the metrics, lower the better. Inference time is tested on one Tesla T4 GPU with a scenario of 50 agents and 150 map elements.}

\centering

    \begin{tabularx}{\textwidth}{l *{4}{>{\centering\arraybackslash}X} | *{2}{>{\centering\arraybackslash}X}}
    \toprule
    \multirow{2}{*}{\shortstack{model}} & minADE$_{1}$ & minFDE$_{1}$ & minADE$_{6}$ & minFDE$_{6}$ & \# model params& inference time\\
        & [m]&[m]& [m] & [m] & [k]& [ms]\\
        \midrule
        \multirow{2}{*}{QCNet \cite{zhou_query_2023}} &0.820 & 2.171 & 0.344& 0.696 &7600& -\\
        &(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(100.0\%)&(-\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        FMAE \cite{cheng_forecast_2023} &0.889 & 2.318& 0.374 & 0.871 & 1900 &-\\
        w/o pre-train&(108.4\%)&(106.8\%)&(108.7\%)&(125.1\%)&(25.0\%)&(-\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        \multirow{2}{*}{EP-Q (ours)} &0.821 & 2.155 & 0.359 & 0.802 & 334 & -\\
        &(100.1\%)&(99.3\%)&(104.4\%)&(115.2\%)&(4.4\%)&(-\%)\\
        \cmidrule(lr){2-5} \cmidrule(lr){6-7}
        \multirow{2}{*}{EP-F (ours)} & 0.831 & 2.171  & 0.370 & 0.825 & 345&-\\ 
        &(101.3\%) & (100.0\%) & (107.6\%) & (118.5\%) &(4.5\%)&(-\%)\\
        \bottomrule
    \end{tabularx}
    \label{tab: in-distribution result wo}
    \vspace{-5pt}
\end{table*}

